A Software-Defined Channel Sounder for Industrial Environments with Fast Time Variance

Novel industrial wireless applications require wideband, real-time channel characterization due to complex multipath propagation. Rapid machine motion leads to fast time variance of the channel's reflective behavior, which must be captured for radio channel characterization. Additionally, inhomogeneous radio channels demand highly flexible measurements. Existing approaches for radio channel measurements either lack flexibility or wide-band, real-time performance with fast time variance. In this paper, we propose a correlative channel sounding approach utilizing a software-defined architecture. The approach enables real-time, wide-band measurements with fast time variance immune to active interference. The desired performance is validated with a demanding industrial application example.

==> ch-meassetup.tex <==
\todo[inline]{Niels}

==> ch-related.tex <==
%%TODO: Channel Sounder using Frank Zadoff Chu sequences
%
%%TODO: Various publications describe the use of FZC sequences in time-variant radio channel measurements:
%%TODO: combine into single text, only most important information!
%
%
%\begin{itemize}
%\item \cite{2011.CaoZhao}
%	\begin{itemize}
%	\item Non-real-time
%	\item SISO measurement
%	\item \unit[625]{MHz} center frequency
%	\item \unit[25]{MHz} bandwidth
%	\item arbitrary waveform generator and real-time spectrum analyzer
%	\end{itemize}
%\item \cite{2016.HolfeldWieruch}
%	\begin{itemize}
%	\item Real-time
%	\item SISO measurement
%	\item \unit[5.85]{GHz} center frequency
%	\item \unit[250]{MHz} bandwidth
%	\item Hardware-defined HIRATE channel sounder introduced by \cite{2013.KeusgenKortke}
%	\end{itemize}
%\item \cite{2016.LvYang}
%	\begin{itemize}
%	\item Real-time channel estimation
%	\item pilot sequences in multi-user (MU) MIMO cellular communication
%	\end{itemize}
%\item \cite{2016.ZhongWu}: 
%	\begin{itemize}
%	\item Non-real-time
%	\item MIMO measurement
%	\item \unit[26]{GHz} center frequency
%	\item \unit[76]{MHz} bandwidth
%	\item hardware not specified in the publication
%	\end{itemize}
%\end{itemize}
%
%%TODO: Even though some hardware-defined channel sounders show superior performance, none of the mentioned publicated measurements satisfy the need for cost-efficient, real-time, software-defined industrial radio channel measurements creating a scalable and flexible measurement system. 
%%TODO: As to the best of our knowledge, no publication combines satisfaction of all described needs. 
%
%%TODO: Channel Sounder using Software Defined Radios
%
%\begin{itemize}
%\item \cite{2009.GahadzaKim}
%	\begin{itemize}
%	\item PN-sequence-based channel sounder
%	\item uses Ettus' first-generation USRP SDRs
%	\item operational bandwidth limited to \unit[4]{MHz} because SDRs were connected using USB, which renders them unfit for measurements of industrial radio channels
%	\end{itemize}
%\item \cite{2012.HwangTsai}
%	\begin{itemize}
%	\item Non-real-time
%	\item Wide bandwidth
%	\item MIMO measurement
%	\item Emulated channel
%	\item Instruments-in-MATLAB Software-Defined Radio
%	\item Realized with separate off-the-shelf measurement instruments for waveform generation, modulation/demodulation and signal storage. 
%	\end{itemize}
%\item \cite{2016.ElofssonSeimar}
%	\begin{itemize}
%	\item Real-time
%	\item MIMO measurement
%	\item With \ac{MLS} and \ac{FZC}
%	\item sing \acp{SDR}, but correlation routine is programmed into the \ac{FPGA}. This makes it more of an \ac{HDR}, because the hardware frontend can not be switched without reprogramming the FPGA.
%	\end{itemize}
%\end{itemize}

%\todo[inline]{\textbf{Computation effort: }
%\\
%"FZC sequence of length P requires P operations to compute" \cite{2009.BeymeLeung}
%\\
%"DFT implemented as FFT reduces the number of arithmetic operations to P log P" \cite{2009.BeymeLeung}
%\\
%"DFT of a FZC sequence of length P can be computed with approximately P operations." \cite{2009.BeymeLeung}}
%
%\todo[inline]{%"it has been proven in \cite{1972.Chu}, that Chu sequences are perfect sequences having an ideal PACF whereas the PCCF for the case that $N$ is odd can be found in ..."
%FZC sequences have an out-of-phase PACF value of zero \cite{1979.Sarwate}}
